The Informativeness of Combined Experimental and Observational Data under Dynamic Selection

This paper addresses the challenge of estimating the Average Treatment Effect on the Treated Survivors (ATETS; Vikstrom et al., 2018) in the absence of long-term experimental data, utilizing available long-term observational data instead. We establish two theoretical results. First, it is impossible to obtain informative bounds for the ATETS with no model restriction and no auxiliary data. Second, to overturn this negative result, we explore as a promising avenue the recent econometric developments in combining experimental and observational data (e.g., Athey et al., 2020, 2019); we indeed find that exploiting short-term experimental data can be informative without imposing classical model restrictions. Furthermore, building on Chesher and Rosen (2017), we explore how to systematically derive sharp identification bounds, exploiting both the novel data-combination principles and classical model restrictions. Applying the proposed method, we explore what can be learned about the long-run effects of job training programs on employment without long-term experimental data.

==> original_slides_related/preambles_for_slides.tex <==

\usepackage{comment}
\excludecomment{en-text}
\usepackage[edges]{forest}
\usepackage{tree}
\usepackage{apalike}
%\usepackage[round]{natbib}
\usepackage[utf8]{inputenc}\usepackage{enumerate}\usepackage{amsmath}\usepackage{amssymb}\usepackage{graphicx}%\usepackage[dvipsnames]{xcolor}
\usepackage{tikz}\usepackage{bm}\usepackage{proof}\usepackage{amsfonts}\usepackage{tcolorbox}\usepackage{ascmac}\usepackage{fancybox}


\usepackage{siunitx}
\let\svqty\qty
\usepackage{physics}
\let\qty\svqty
\usepackage{hyperref}
\hypersetup{
    colorlinks,
    citecolor=black,
    filecolor=black,
    linkcolor=black,
    urlcolor=black
}
\newtheorem{definitionOfMine}{Definition}[section]
\newtheorem{mytheorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem*{remark}{Remark}
\newtheorem*{lemma*}{Lemma}
\newtheorem{assumption}{Assumption}[section]
\newtheorem{notation}{Notation}[section]
\newtheorem{algorithm}{Algorithm}[section]

\setbeamertemplate{theorems}[numbered]
\newtheorem{innercustomthm}{Condition}
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
  
\newtheorem{mycorollary}{Corollary}[section]

\newcommand{\koko}{{\color{yellow}koko}}
\newcommand{\todo}{{\color{red}todo}}
\newcommand{\qu}{{\color{green}queue}}
\newcommand{\yp}[1]{\textcolor{blue}{Park: #1}}

%%% added by Hirofumi Shiba 10/27/2022
\AtBeginDocument{\RenewCommandCopy\qty\SI} 
\newcommand{\mathrf}[1]{\mathrm#1}
\newcommand{\Abs}[1]{\left|#1\right|}\newcommand{\Norm}[1]{\left\|#1\right\|}\newcommand{\Brace}[1]{\left\{#1\right\}}\newcommand{\paren}[1]{\left(#1\right)}\newcommand{\bracket}[1]{\langle#1\rangle}\newcommand{\brac}[1]{\langle#1\rangle}\newcommand{\Bracket}[1]{\left\langle#1\right\rangle}\newcommand{\Brac}[1]{\left\langle#1\right\rangle}\newcommand{\Square}[1]{\left[#1\right]}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\sub}{\subset}
\DeclareMathOperator*{\esssup}{ess\,sup}

\newcommand{\X}{\mathcal{X}}\newcommand{\V}{\mathcal{V}}
\newcommand{\F}{\mathfrak{F}}\newcommand{\Om}{\Omega}\newcommand{\om}{\omega}\newcommand{\R}{\mathbb{R}}\renewcommand{\P}{\mathbb{P}}
\newcommand{\ifquad}{\text{if}\quad}
\newcommand{\Sel}{\mathrm{Sel}}
\newcommand{\as}{\text{a.s.}}

\usepackage{graphicx}
\usepackage{xspace}
%\usepackage{bxdpx-beamer}
\usepackage{amsmath}
%\usepackage[at]{easylist} 
\usepackage{ascmac}
\usepackage{mathtools}
\usepackage{here}
\usepackage{comment}
\usepackage{arydshln} % \hdashline
\usepackage{bm}
\usepackage{caption}
\usepackage{appendixnumberbeamer}
\usepackage{CJKutf8}
\usepackage{multirow}
\usepackage{tikz}


\AtBeginSection[]{
  \begin{frame}
  \vfill
  \centering
  \begin{beamercolorbox}[sep=8pt,center,shadow=true,rounded=true]{title}
    \usebeamerfont{title}\insertsectionhead\par%
  \end{beamercolorbox}
  \vfill
  \end{frame}
}

\setbeamercovered{transparent} 


\usepackage{xcolor}
\hypersetup{
	colorlinks=false,
	citebordercolor=green,
	linkbordercolor=red,
	urlbordercolor=cyan,
}

% Japanese: platex
%\usepackage{pxjahyper} % しおりの和文対応
%\usepackage{minijs} %和文用
%\renewcommand{\kanjifamilydefault}{\gtdefault} % 日本語フォントの設定
%\usepackage[deluxe, expert]{otf} %日本語フォント

% Themes
%\usetheme[progressbar=frametitle]{metropolis}
%\usetheme{Boadilla}
\usetheme{Singapore}
%\usetheme{Montpellier}
%\useoutertheme{}
%\useinnertheme{}
%\usefonttheme{}
\usecolortheme{rose}

\setbeamercolor{frametitle}{fg=royalblue}
\setbeamercolor{framesubtitle}{fg=royalblue2}
%,bg=Brown!20

% Fonts
\usepackage[sfdefault]{noto} % DejaVu Sans
\usepackage[T1]{fontenc}
\usefonttheme{professionalfonts} % Font for equations

\setbeamertemplate{navigation symbols}{} % ナビゲーションシンボルの消去
\setbeamertemplate{navigation tree}{}
\setbeamertemplate{footline}[frame number]
\setbeamerfont{frametitle}{size=\Large}
\setbeamerfont{framesubtitle}{size=\large}
\setbeamerfont{caption}{size=\normalsize} %キャプションサイズ
%\AtBeginSection[]
%	{\begin{frame}[shrink]{Outline}
%		\tableofcontents[currentsection, hideothersubsections]
%	\end{frame}}
%\usepackage[absolute,overlay]{textpos}
%\setbeamercovered{transparent}

% Define colors
\definecolor{mex}{RGB}{67, 135, 233}
\definecolor{themecolor}{RGB}{0,0,50} 
\definecolor{alertred}{RGB}{210,0,0} 
\definecolor{darkblue}{RGB}{0,0,150}
\definecolor{lightblue}{RGB}{0,0,50}
\definecolor{mossgreen}{RGB}{0,150,0} 
\definecolor{chocobrown}{RGB}{75,50,50} 
\definecolor{gray}{RGB}{180,180,180}
\definecolor{skyblue}{RGB}{0,100,150}
\definecolor{burgundy}{RGB}{180,30,30}
\definecolor{royalblue}{RGB}{65,105,225}
\definecolor{royalblue2}{RGB}{65,105,225}
\definecolor{gold}{RGB}{140,140,0}

% Set default colors
\setbeamercolor{structure}{fg=black}
\setbeamercolor{alerted text}{fg=gold}
\setbeamercolor{example}{fg=mossgreen}

% ブロック環境のフチを丸く、影をつける
\setbeamertemplate{blocks}[rounded]%[shadow=true]

% Reduce indent in itemize
% \setlength{\leftmargini}{0.55cm}
% \setlength{\leftmarginii}{0.4cm}
% \setlength{\labelsep}{0.1cm}

% ToC
\setbeamertemplate{section in toc}[sections numbered]
\setbeamertemplate{subsection in toc}[subsections numbered]
%\setbeamertemplate{subsection in toc}
%{\leavevmode\leftskip=2em\rlap{\hskip-2em$\quad$\inserttocsectionnumber.\inserttocsubsectionnumber}$\quad$\inserttocsubsection\par}

% Itemize/enumerate environment
%\setbeamertemplate{itemize items}[square]
\setbeamertemplate{itemize subitem}{--}
\setbeamertemplate{itemize subsubitem}{\checkmark}
%\setbeamertemplate{enumerate items}{(\alph{enumi})}
%\setbeamertemplate{enumerate subitem}{(\roman{enumii})}
%\setbeamertemplate{enumerate subsubitem}{(\roman{enumiii})}


\setbeamertemplate{frametitle continuation}[from second][(contd.)]

% Faded overlay
\newcommand<>{\uncovergraphics}[2][{}]{
	% Taken from: <https://tex.stackexchange.com/a/354033/95423>
	\begin{tikzpicture}
		\node[anchor=south west,inner sep=0] (B) at (4,0)
		{\includegraphics[#1]{#2}};
		\alt#3{}{%
			\fill [draw=none, fill=white, fill opacity=0.7] (B.north west) -- (B.north east) -- (B.south east) -- (B.south west) -- (B.north west) -- cycle;
		}
	\end{tikzpicture}
}

% Others
\def \blue #1{\textcolor{royalblue}{#1}} %blue
\def \blueu #1{\textcolor{royalblue}{\underline{#1}}} %blue
\def \red #1{\textcolor{alertred}{#1}} %blue
\def \redu #1{\textcolor{alertred}{\underline{#1}}} %blue
\def \green #1{\textcolor{mossgreen}{#1}} %blue
\def \greenu #1{\textcolor{mossgreen}{\underline{#1}}} %blue
\def\v#1{\mbox{\boldmath $#1$}} %ベクトル
\newlength{\mytotalwidth}
\mytotalwidth=\dimexpr\linewidth-5mm
\newlength{\mycolumnwidth}
\mycolumnwidth=\dimexpr\mytotalwidth-5mm

\newcommand{\re}{\mathbb{R}}
\newcommand{\ex}{\mathrm{E}}


